Layer-Neighbor Sampling -- Defusing Neighborhood Explosion in GNNs

Graph Neural Networks (GNNs) have received significant attention recently, but training them at a large scale remains a challenge. Mini-batch training coupled with sampling is used to alleviate this challenge. However, existing approaches either suffer from the neighborhood explosion phenomenon or have poor performance. To address these issues, we propose a new sampling algorithm called LAyer-neighBOR sampling (LABOR). It is designed to be a direct replacement for Neighbor Sampling (NS) with the same fanout hyperparameter while sampling up to 7 times fewer vertices, without sacrificing quality. By design, the variance of the estimator of each vertex matches NS from the point of view of a single vertex. Moreover, under the same vertex sampling budget constraints, LABOR converges faster than existing layer sampling approaches and can use up to 112 times larger batch sizes compared to NS.

==> icml_rebuttal.tex <==
Main rebuttal:

We thank all the reviewers for their valuable feedback.

Test accuracies:

We will add below listed test accuracies to Table 2.
We would like to stress that no hyperparameter tuning was performed, all hyperparameters were fixed for 
all datasets except for LADIES variants whose sampled vertex numbers were picked to match LABOR-* on each dataset as 
can be in Table 2.

|        | reddit        | products      | yelp          | flickr       |
|--------|-------------- |---------------|---------------|--------------|
|PLADIES | 96.21 +- 0.06 | 78.44 +- 0.24 | 61.55 +- 0.87 | 51.52 +- 0.26|  
|LADIES  | 96.20 +- 0.05 | 78.59 +- 0.22 | 61.89 +- 0.66 | 50.79 +- 0.29*|  
|LABOR-* | 96.23 +- 0.05 | 78.59 +- 0.34 | 61.57 +- 0.67 | 51.67 +- 0.27|  
|LABOR-1 | 96.23 +- 0.06 | 78.47 +- 0.26 | 61.71 +- 0.70 | 51.66 +- 0.24|  
|LABOR-0 | 96.25 +- 0.05 | 78.76 +- 0.26 | 61.55 +- 0.85 | 51.65 +- 0.26|  
|NS      | 96.24 +- 0.05 | 78.48 +- 0.29 | 61.50 +- 0.66 | 51.70 +- 0.23|  

As seen in the results, all accuracies are within one standard deviation of
each other except for LADIES on flickr, which we highlighted with a star. They perform the same because we chose their
hyperparameters fairly, i.e., we picked the same fanout values for LABOR and NS, and for LADIES variants we made sure to
sample the same number of vertices as LABOR-*. Then, the real question is, why would we use one over the other?

The answer to which sampler to use is embedded in Table 2, in the $|V_l|$ and $|E_l|$ columns. These columns give us
the number of vertices and edges sampled in the $l$-th layer with the last layer, the last layer ($|V_3|$ and $|E_3|$) being the most important.
Obviously, runtime is a monotonic function of $|V_l|$ and $|E_l|$ and the smaller they are, the faster the training will be.
Different importance (contribution to computational complexity) of $|V_l|$ vs $|E_l|$ would change based on the model. 
Thus, looking at the results, we conclude that that if $|V_l|$ is important, one can use LABOR-* and 
if $|E_l|$ is important (for example, in the GAT model), one can use LABOR-0 to get the best runtime performance.

GAT runs:

During the limited rebutal time we had, we also ran preliminary experiments using the GAT model,
comparing LABOR-0 to NS with the same setup in Figure 1 and Table 2.
Again, same fixed hyperparameters were used, the number of attention head was picked as 4. We computed test
accuracies after training on random neighbors of 30 using NS, otherwise we were getting Out-of-Memory (OOM) for some
datasets with full neighborhoods. LABOR-0 was run around 20 times while NS was run around 10 times due to
NS being slower than LABOR-0, average accuracies and runtime per iteration on NVIDIA A100 is being reported.
LADIES variants were too slow in this experiment due to it sampling too many edges on the reddit and products 
datasets, and it ran OOM during most of our runs. This is due to the fact that GAT is implemented via an 
Sampled Dense-Dense Matrix Multiplication operation, and matrices whose number of rows is the sampled number of
edges being computed. Thus, memory and runtime requirements of the GAT model strongly correlate with the number of sampled edges.

|        |  reddit                | products               | yelp                  | flickr               |  
| ------ | ---------------------- | ---------------------- | --------------------- | -------------------- |  
|LABOR-0 | 95.28 +- 0.11, 57.1ms  | 80.18 +- 0.39, 138.5ms | 54.24 +- 0.35, 82.9ms | 54.19 +- 0.26, 72.6ms|  
|NS      | 95.51 +- 0.52, 166.8ms | 79.62 +- 0.51, 218.7ms | 54.32 +- 0.51, 99.6ms | 53.99 +- 0.38, 77.1ms|  

We invite the reviewers to compare the GAT runtime numbers to Table 2, $|E_3|$ column to see the correlation. We
see that LABOR fills an important gap in the literature as an edge efficient layer sampler (LABOR-0).

Dear reviewer 1qQw

Thank you very much for the feedback. We will take it into account and work on improving the clarity of our presentation. Before that, we would like to address the questions and issues brought up below:

Question 1: We defined $M_t := H_t W$ to denote the messages along each edge. Since $W$ is changing during training 
and our framework doesn't make use of the embedding magnitudes $|H_t W|$ like AS-GCN does, we make the simplifying 
assumption $E[|M_t|] = E[|M_{t'}|] \forall t, t' \in V$. To further simplify the analysis, we further assume that
$Var(M_t) = 1, \forall t \in V$, here the variance comes from the fact that $M_t$ evolves during training with 
changing model parameters and also the fact that $M_t$ will be computed as a result of random sampling in the next 
layer. We derive all the equations later in the text with these assumptions.  
Thus we focus on sampling of a single layer independently of others, since we don't assume anything about $Var(M_t)$ 
or $E[|M_t|]$ for different $t$ as they are unknown and are results of a random and time evolutionary process,
so our analysis treats them uniformly. Our results show that this analysis works, LABOR variants seem 
to match each other and NS in terms of convergence behaviour plotted with respect to the training iterations in 
Figure 3. The provided test accuracy numbers in our main rebuttal prove that this is the case as well.

Follow-up:
We thank the reviewer for the follow-up.

We believe that we have answered Question 1.1 by stating our assumptions about uniform embedding magnitudes $E[|M_t|]$ and uniform embeddings variances $Var(M_t)$.  We have also explained that messages along each edge $M_t$ is a time changing random variable due to changing model weights and random sampling over multiple layers.

We also gave a complexity analysis for our algorithm and its pseudocode, resolving Question 1.4.

For Questions 1.2 and 1.3, we would like to make clear that the Hajek estimator in eqn. (7) can be used with either of Poisson Sampling, Sampling without replacement or Sampling with replacement. In what follows, we fix the vertex $s$ and we assume $Var(M_t) = 1, \forall t \in N(s)$ and $E[|M_t|] = \frac{1}{d_s}, \forall t \in N(s)$. Eqn. (8) gives the variance of Hajek estimator for sampling without replacement, for verification you can look at Eqn. (3.13) in [1] and for a derivation, please see [2] page 8 SRSWOR section. In Eqn. (10), we set the variance target for each vertex to $\frac{1}{k} - \frac{1}{d_s}$ for Poisson Sampling. Setting $\pi_t = \frac{k}{d_s}$ makes Poisson Sampling have the set variance target, $\frac{1}{d_s^2}\sum_{t \to s} \frac{1}{\frac{k}{d_s}} - \frac{1}{d_s} = \frac{1}{d_s^2} d_s \frac{d_s}{k} - \frac{1}{d_s} = \frac{1}{k} - \frac{1}{d_s}$.

Since we set $\tilde{d_s} = k$, the variance of sampling without replacement is $\frac{d_s - k}{d_s - 1}\frac{1}{k}$.  Subtracting these two variances in Eqn. (11), we see that it is negative.

To verify that the left-hand side of Eqn. (10) is the variance of Poisson Sampling, we invite you to take a look at [3] Eqn. 3 (Since we are taking the mean, $E[|M_t|]^2 = y_i^2 = \frac{1}{d_s^2}$). For example, the variance of the Hajek estimator for Sampling with replacement would be $\frac{1}{k}$, worse than both Poisson Sampling and sampling without replacement.

[1] https://www.ph.ucla.edu/epi/rapidsurveys/RScourse/RSbook_ch3.pdf  
[2] http://home.iitk.ac.in/~shalab/sampling/chapter2-sampling-simple-random-sampling.pdf  
[3] Williams, M. S., Schreuder, H. T., and Terrazas, G. H. Poisson Sampling – The Adjusted and Unadjusted Estimator Revisited. pp. 12, 1998

One more follow-up:

We ran a numerical experiment in the equal probability case to verify whether the variances of Poisson Sampling, Sequential Poisson Sampling, Sampling without replacement and Sampling with replacement match the formulas we claimed.

Code: https://colab.research.google.com/drive/1G7cqZ7pUD7nSkiVOSkkYEwfF6QT8uxzt?usp=sharing

We saw that Sequential Poisson Sampling and Sampling without replacement have equal variances $(\frac{1}{k} - \frac{1}{d_s}) \frac{d_s}{d_s - 1}$, where $\frac{d_s}{d_s - 1}$ is a correction factor ([4], remark 2.1) for the variances of Poisson Sampling variants. With this correction factor, its variance is equal to the claimed variance of sampling without replacement $\frac{d_s - k}{d_s - 1}\frac{1}{k}$. We also noticed that the variance of Poisson Sampling is a little higher compared to Sequential Poisson Sampling and Sampling without replacement, the difference grows as $k$ and $d_s$ become smaller but vanishes as $k$ and $d_s$ tend to infinity. This is due to the fact that Poisson Sampling can sample different number of items each time it is invoked, as explained in [4]. Sequential Poisson Sampling doesn't have this problem.

Thus, we will update Eqn. (9) by multiplying the right-hand side with $\frac{d_s}{d_s - 1}$, and we will update our paper to clarify that we are using the approximate variance formula for Poisson Sampling, and its variance is not strictly lower than sampling without replacement but is approximately equal. When one uses Sequential Poisson Sampling, then their variances become exactly equal in the equal probability case. We will also scale our variance target $\frac{1}{k} - \frac{1}{d_s}$ by the same correction factor $\frac{d_s}{d_s - 1}$, in which case the equalities in Eqn. (10, 14) don't get affected at all since both sides are scaled with the same factor.

We thank the reviewer for noticing this mistake and we will fix our wording to reflect this new finding. It is nontrivial to calculate the exact variances for these different sampling methods so some of the formulas we took from papers in the statistics community were approximate, leading to this minor mistake.

Poisson Sampling is very simple. For each edge, we can flip a coin to decide whether to sample it. This can easily be achieved with a parallel copy_if algorithm, which is available in NVIDIA's thrust library, which we utilized in our GPU implementation. Parallel Sequential Poisson Sampling can be implemented with a parallel segmented sorting algorithm, however the overhead of parallel segmented sorting was not enough to justify the small variance benefit it brings over Poisson Sampling.

[4] Esbjorn Ohlsson, Sequential Poisson Sampling, 1998, https://www.scb.se/contentassets/ca21efb41fee47d293bbee5bf7be7fb3/sequential-poisson-sampling.pdf

Question 2: For a vertex $s$, NS samples $\min(k, d_s)$ neighbors deterministically. Our poisson approach samples $\min(k, d_s)$ vertices in expectation. If sequential poisson sampling is used, our approach sampled $\min(k, d_s)$ vertices deterministically matching the behaviour of NS.

Question 3 and the Limitations: We would like to note that the overhead cost of computing each iteration of $c$ and 
$\pi$ is a sparse matrix times vector multiplication (SpMV) using the E ($E = |\{t \to s \mid s \in S\}|$) edges 
$O(E)$. Note that cuSparse library by NVIDIA provides efficient SpMV algorithms for their GPUs.
Once $c$ and $\pi$ are determined in $i$ iterations for LABOR-i algorithm, the sampling cost is $O(E)$. Thus 
the runtime complexity of NS and LABOR variants are equivalent. Not 
only that, all these operations are easily parallelizable, to prove that, we provide an anonymized notebook running
a GPU implementation of LABOR along with NS.  
Link to runnable code: https://colab.research.google.com/drive/1NAv2F6-eeiYsLrnSVPTBKSRMOJOVti6m?usp=sharing  
We are also including the sampled number of vertices and the standard deviation values for the Yelp dataset here:  
```
Sampler: LABOR-3, mean: [106979.32], std: [1619.06], average GPU time in ms: 18.18  
Sampler: LABOR-0, mean: [140526.18], std: [2073.41], average GPU time in ms: 7.77  
Sampler: NS, mean: [190292.78], std: [2505.03], average GPU time in ms: 6.32  
```
One can see that the use of Poisson sampling doesn't cause any more randomness in terms of memory use as the variance 
in the numbers don't look any different compared to NS and also that LABOR is parallelizable on the GPU,
as also shown in the Table 2 in the it/s column on an NVIDIA T4 GPU.

Question 4: We will add a full description of the sampling procedure in the form of a pseudocode for the camera-ready version. A pseudocode for LABOR assuming uniform edge weights looks as follows:

```
Inputs to Labor:
S is a set of seed vertices
i denotes that we will use LABOR-i
k is the fanout value

T = \{ t | t \in N(S) \}
Initialize \pi_t = 1 for all t \in T

while i > 0:
  for s in S:
    Solve Equation (14) for c_s
  for t in T:
    \pi_t = \pi_t * \max_{t \in N(s)} c_s
  i = i - 1

Initialize r_t = U(0, 1) for all t \in T
sampled_edges = []
sampled_importance_weights = []
for s in S:
  normalize_pi = 0
  for t in N(s):
    if r_t <= c_s \pi_t:
      sampled_edges.append((t -> s))
      normalize_pi = normalize_pi + 1 / \pi_t
  for t in N(s):
    if r_t <= c_s \pi_t:
      sampled_importance_weights.append((1 / \pi_t) / normalize_pi)

return sampled_edges, sampled_importance_weights
```

In the above algorithm, sampled_edges and sampled_importance_weights arrays are of the same length and they are
used to evaluate the Hajek estimator for each vertex s, similar to Equation (5). Also, all parts of our algorithm
can be made parallel and run on GPUs.

Dear reviewer 8Kz1

Thank you very much for the feedback. Before we implement your suggestions for the camera-ready version, we would like to address some of the weaknesses you brought up.

Weakness 1: For the camera-ready version, we will work on a theoretical discussion on the estimation errors of LADIES and LABOR. We will also include empirical results, e.g., freezing model weights after training and measuring the variance of the estimations of the initial seed vertices along with the variance of $\tilde{d_s}$ in a multi-layer GNN model over different sampled multi-layer neighborhoods to test our hypothesis.

Weakness 2: We will make it more clear why LABOR is faster than NS in terms of it/s. It is because it samples fewer vertices and edges, which translates into a runtime speedup. If we look at Table 2, we can see that on reddit, LABOR-0 samples 5x fewer vertices than NS, and thus the it/s is 37.6 vs 14.2 respectively. The number of sampled vertices and edges determines how much work needs to be performed to process a single iteration.

Weakness 3: We will cite the GAS and LMC methods you point to in addition to other papers we will find meanwhile. In addition, please feel free to point out other references you think are relevant.

Weakness 4: Thanks for the suggestion. We will modify the figures to include a zoom into the regions where the better algorithms compete. The differences will be clear to see as a result.

Questions: LABOR-0 can be used as a drop-in replacement to NS in any scenario, so given a working NS implementation 
for any aggregator, one can swap it out for LABOR-0. However when it comes to importance sampling, it is necessary to 
do a complete new analysis.
Even if one attempted to use NS or LABOR-0 for the max aggregator, it will be necessary to do some degree based 
scaling to make the sampling unbiased similar to Section 2.2 of PNA [3].
The scaling would depend on the aggregator in use, for example sum and max would need to use different degree based 
expressions for the scaling. We will think about different aggregators more and include a discussion on them for the 
camera-ready version. While an unbiased scaling factor for the sum aggregator would be very simple to derive
(just scale by $d_s$, as our paper uses the mean aggregator), we currently don't know what exact form the scaling 
factor would take for the max operator. We will that this analysis along with feasibility of importance sampling
deserves its own write-up.


Dear reviewer tDhZ

Thank you very much for your feedback.

Comments on pointed out weaknesses:
* After your suggestion, we did an initial experiment comparing NS to LABOR-0 using the GAT model. Please take a look at
our main rebuttal, GAT runs section.
* We have included a limited comparison against GraphSAINT edge sampler in Appendix A.4.
Shadow is a meta sampling algorithm and takes another
sampler as its EXTRACT algorithm. It is possible to use any LABOR variant as the EXTRACT method for SHADOW. Thus, we
didn't feel the need to compare against it as SHADOW and LABOR are complementary algorithms to each other.
The reason we didn't
include subgraph sampling algorithms in our main experimental evaluation is to highlight the similarities and 
differences between the existing neighbor and layer sampling methods to the ones we proposed.
* We will include additional experiments to measure the variance of estimators of LABOR and LADIES in the output layer in 
the multi-layer setting. The main problem with LADIES is that it assumes the next layer vertex embeddings have equal 
variance when it performs importance sampling. However, due to the fact that it is possible for it to sample drastically 
different number of edges for each vertex it samples in the previous layer, the equal variance assumption doesn't hold at 
all. However, since LABOR samples the same number of edges for each vertex in the next layer, the equal variance
assumption holds more for LABOR especially in the multi-layer setting.
That is why LABOR outperforms LADIES overall. We are currently working on an experiment to measure the variance in the 
output embeddings of LABOR and LADIES, we are hoping that its results will support our claim, we might be able to provide
preliminary results during the reviewer-author discussion period.
* Yes, it is marginal. That is because we are fixing a bias in LADIES' construction that doesn't surface in every
scenario, but it did seem to show up on the Flickr dataset. We suspect that this is due to the fact that Flickr dataset
has the smallest average degree among all the datasets, exacerbating the bias of LADIES.
* We will modify the plots to include a zoom into the regions where the better algorithms compete. The differences will be clear to see as a result. We will also consider using a log axis as you suggested, whichever approach better reflects the differences.
* We have modified our paper to include test accuracies in Table 2 (corresponds to Figure 1) and included them in our 
main rebuttal. The experiment in Figure 2 was to highlight the sampling efficiency under a given budget. Nobody
actually trains GNN models with a 10000 batch size (Table 3) on the Reddit dataset.

Responses to questions:
* Cluster-GCN is a biased subgraph sampling method as the edges inside the clusters are sampled more often than edges
across clusters. However, other most of the other subgraph sampling methods in the literature are designed to be 
unbiased. We will clarify it in our paper. Subgraph sampling methods were not compared against in the main text
to focus on layer and neighbor sampling algorithms, saving space for a more detailed investigation. Appendix A.4
has a limited comparison against GraphSAINT.
* Right after equation 6 in the paper, we say that we assume the variances $Var(M_t)$ are equal to $1$. Thus, the variance
of the Hajek estimator becomes the same as the variance of sampling i.i.d items without replacement, with the first
fraction in (8) being the Finite Population finite population correction (FPC) factor. This is discussed in the following
link in more detail: https://www.ph.ucla.edu/epi/rapidsurveys/RScourse/RSbook_ch3.pdf.
* Minibatching is carried out by
shuffling the training vertices prior to every epoch and choosing consecutive $B$ elements as the seed vertices of the
minibatch every iteration. Then the minibatch is formed by recursively sampling the one hop neighborhood of these seed
vertices for every layer (the output of one layer becomes the seed vertices of the next). In the proposed sampling 
algorithms, PLADIES and LABOR, there is mathematically no bias at all by construction except for any bias introduced
by the Hajek estimator (Equation (4)) compared to Thompson-Horvitz (Equation (5)). However, the vertex sampling
probabilities and procedure of LABOR and PLADIES are fully unbiased.


Dear reviewer ih5t

Thank you very much for your feedback.

Taking your feedback into account, we added the test accuracy results corresponding to the experiment in Figure 1 to 
Table 2 as a separate column, please take a look at the test accuracy section in our main rebuttal. Initially, we 
left out the test accuracy results as we didn't do any hyperparameter tuning, you can see that we use the same 
hyperparameters for all the datasets.

Since the review period is limited and GAT model running slower, we have some preliminary results in our main 
rebuttal, GAT runs section. However, full results should be ready for the camera ready version if you favor our paper 
and it gets accepted, in which case the final paper will include GAT results. Since the GCN results are so close to 
each other, we expect GAT results to be similar, and our preliminary results show that accuracies of LABOR-0 and NS
are almost the same, except for runtime difference favoring LABOR-0 heavily.

Finally, our Appendix A.4 has some comparison against GraphSAINT in terms of time taken to converge to a given 
accuracy target and LABOR and NS variants seemed to outperform GraphSAINT there. In our opinion, as the graph becomes 
larger and larger and the batch size stays fixed, we theorize that the following will happen: Subgraph sampling 
methods similar in construction to GraphSAINT sample vertices/edges independently, thus as the graph size tends to
infinity, the number of edges in the sampled subgraph will tend to 0. Hence, we think that GraphSAINT will not scale. 
Cluster-GCN  method is a biased method since it creates clusters and samples vertices
belonging to the same cluster together. In this paper, our goal was to investigate unbiased sampling methods and also 
limit the problem space by assuming no knowledge of vertex embedding distribution so that we can focus the discussion 
on the main limitations of LADIES and NS. Also, we think that this kind of discussion can be left as future work as 
our main focus was non-subgraph sampling methods.

Another subgraph sampling method is SHADOW (Decoupling the Depth and Scope of Graph Neural Networks), that uses
a given sampler such as NS or any LABOR variant as the EXTRACT method and generates an $L$-hop neighborhood. Then,
with appropriate unbiasing measures, they use the extracted subgraph and perform training with a model with more
than $L$ layers. Note that, even though it is a subgraph sampling method, it is actually uses the $L$-hop neighborhood
of the given seed vertices unlike GraphSAINT or Cluster-GCN. Also, since it is a meta method, meaning that EXTRACT
can be any sampler, it can actually be enhanced by the use of LABOR-0 instead of NS algorithm they use in their
experiments, enjoying the same benefits we show in our paper. 

One can see that the GNN sampling literature has chosen NS as their defacto sampling algorithm, our goal is to change 
that to LABOR-0 (It is used as a direct drop-in) in this paper. Some example papers, that we have cited in our paper,
almost explicitly using NS as their samplers:

VR-GCN: Stochastic training of graph convolutional networks with variance reduction
SHADOW: Decoupling the Depth and Scope of Graph Neural Networks
GNS: Global Neighbor Sampling for Mixed CPU-GPU Training on Giant Graphs
BS: Bandit samplers for training graph neural networks
Thanos: A Biased Graph Neural Network Sampler with Near-Optimal Regret

All the papers above can be improved just by switching NS with LABOR-0, we are hoping that you are convinced at this
point that LABOR-0 outperforms NS in terms of efficiency while matching its quality.
